COP: Control & Observability-aware Planning

In this research, we aim to answer the question: How to combine Closed-Loop State and Input Sensitivity-based with Observability-aware trajectory planning? These possibly opposite optimization objectives can be used to improve trajectory control tracking and, at the same time, estimation performance. Our proposed novel Control & Observability-aware Planning (COP) framework is the first that uses these possibly opposing objectives in a Single-Objective Optimization Problem (SOOP) based on the Augmented Weighted Tchebycheff method to perform the balancing of them and generation of B\'ezier curve-based trajectories. Statistically relevant simulations for a 3D quadrotor unmanned aerial vehicle (UAV) case study produce results that support our claims and show the negative correlation between both objectives. We were able to reduce the positional mean integral error norm as well as the estimation uncertainty with the same trajectory to comparable levels of the trajectories optimized with individual objectives.

==> 210_control.tex <==
We now recall the main notions behind the definition of the closed-loop state and input sensitivities which have been introduced in~\cite{robuffo_sensitivity_2018,brault_robust_2021}.

Consider a generic robot model
\begin{equation}\label{eq:system}\small
\dot{\vx}  =  \vf(\vx,\,\vu,\,\vp)
\end{equation}
where $\vx\in\mathbb{R}^{n_x}$ is the state vector, $\vu\in\mathbb{R}^{n_u}$ is the control input vector, and $\vp\in\mathbb{R}^{n_p}$ the vector of \emph{system} parameters (which are assumed uncertain). Consider also a generic control law
\begin{equation}\label{eq:ctrl}\small
\left\{\begin{array}{rcl}
\dot{\bm{\xi}} &=&\vg(\bm{\xi},\,\vx,\,\bm{r}_d(\va,\,t),\,\vp_c) \vspace{5pt} \\ 
\vu&=&\vc(\bm{\xi},\,\vx,\,\bm{r}_d(\va,\,t),\,\vp_c)
\end{array}\right.,
\end{equation}
where $\bm{\xi}\in\mathbb{R}^{n_\xi}$ are the internal controller states (for example an integral action), $\vp_c$ a nominal value for the parameters $\vp$, and $\bm{r}_d(\va,\,t)$ a desired trajectory to be tracked parametrized by vector $\va$ and time $t$. 

\subsection{Sensitivity Metrics}

The state sensitivity matrix is defined as
\begin{equation}
\label{eq:Pi}
\left.
\vPi(t) = \dfrac{\partial  \vx(t)}{\partial \vp}
\right|_{\vp = \vp_c}
\in \mathbb{R}^{n_x \times n_p}
\end{equation}
and it represents the variation of the states with relation to variations in the parameter vector $\vp$, evaluated on the \textit{nominal} value $\vp = \vp_c$. 

The input sensitivity matrix is defined as
\begin{equation}
\left.
\bm{\Theta}(t) = \dfrac{\partial \vu(t)}{\partial \vp}
\right|_{\vp = \vp_c}
\in \mathbb{R}^{n_u \times n_p}
\label{eq:Theta}
\end{equation}
and, similarly to \equref{Pi}, it maps how variations in the parameters result in variations of the control inputs. 

In general, it is not possible to compute $\bm{\Pi}(t)$ or $\bm{\Theta}(t)$ in closed-form. However, it is possible to obtain a closed-form expression for the dynamics of $\bm{\Pi}(t)$ from which any other needed quantity can be computed. For the sake of readability, let us introduce the notation $\bm{x}_{,\bm{y}}$ to refer to the jacobian of a vector function $\bm{x}$ with relation to one of its arguments $\bm{y}$. With this shorthand form, one can show that%~\cite{robuffo_sensitivity_2018,brault_robust_2021}
% \begin{equation}
% \bm{\dot{\Pi}}(t) = \dfrac{\partial \vf}{\partial \vx}\bm{\Pi} + \dfrac{\partial \vf}{\partial \bm{u}}\bm{\Theta} + \dfrac{\partial \vf}{\partial \bm{p}}, \qquad \bm{\Pi}(0) = 0.
% \label{eq:dPi}
% \end{equation}
% For the sake of readability, let us introduce the notation $\vx_{,\bm{y}}$ in order to refer to the jacobian of a vector function $\vx$ w.r.t. one of its arguments $\bm{y}$. With this shorthand, one can show that~\cite{robuffo_sensitivity_2018,brault_robust_2021}  %the set of differential equations to integrate $\bm{\Pi}, \, \Pi_{\bm{\xi}}$ and $\bm{\Theta}$ is
\begin{equation}
\left\lbrace\begin{aligned}
\bm{\dot{\Pi}}(t) &= \vf_{,\vx}\bm{\Pi}(t) + \vf_{,\vu}\bm{\Theta}(t) + \vf_{,\vp}, \quad &\bm{\Pi}(0) = 0,\\
\bm{\dot{\Pi}_{\bm{\xi}}}(t) &= \vg_{,\vx}\bm{\Pi}(t) + \vg_{,\bm{\xi}}\bm{\Pi}_{\bm{\xi}}(t),  &\bm{\Pi}_{\bm{\xi}}(0) = 0,\\
\bm{\Theta}(t) &= \vc_{,\vx}\bm{\Pi}(t) + \vc_{,\bm{\xi}}\bm{\Pi}_{\bm{\xi}}(t)
\end{aligned}\right.
\label{eq:integration1}
\end{equation}
where 
\begin{equation}
\left.
\vPi_{\bm{\xi}}(t) = \dfrac{\partial  \bm{\xi}(t)}{\partial \vp}
\right|_{\vp = \vp_c}
\in \mathbb{R}^{n_{\xi} \times n_p}
\label{eq:Pi_xi}
\end{equation}
represents the control state sensitivity matrix (in general only needed for evaluating the other terms of interest).
%
Therefore, the evolution of ${\vPi}(t)$ over a time interval of interest can be obtained by numerically integrating \equref{integration1} over time, which makes $\bm{\Theta}(t)$ computable as well (note that the various terms in \equref{integration1} depend, in general, on the full state vector $\vx$, therefore an accurate knowledge of the robot state is needed). Note that the evaluation of ${\vPi}(t)$ and $\bm{\Theta}(t)$ is done by leveraging both the robot's model \equref{system} and the control law \equref{ctrl}, so that any strength/weakness of the chosen control action is correctly taken into account. This is why these quantities are also called \emph{closed-loop} state and input sensitivities, since they are evaluated on the full closed-loop system.

\subsection{State and Input-sensitive Optimization}
\label{sec:sis}

Once the quantities $\vPi(t)$ and $\bm{\Theta}(t)$ are available {through numerical integration over the whole trajectory $\bm{r}(\va,\,t)$}, one may use them to formulate a trajectory optimization problem aimed at minimizing the state and input sensitivities by acting on the shape of the desired trajectory $\bm{r}_d(\va,\,t)$. %In particular in~\cite{brault_robust_2021} we proposed to consider the following optimization problem
Consider the following optimization problem
%To enhance the global performance of a robot, we can consider the following problem: knowing our system dynamics $\vf$, a reference path $\bm{r}_d(\bm{a},t)$ defined over the time interval $\mathbb{T}$, the controller internal dynamics $\bm{g}$ and its input function $\bm{h}$, the optimization consists in finding the optimal shape $\bm{a}_{opt}$, such that
\begin{equation}
\label{eq:opt1}
\bm{a}_{opt} = \arg \, \underset{\bm{a} \in \mathcal{A}}{\min}\ \left( w_1 || \bm{\Pi}(T)|| + w_2 \int_0^T || \bm{\Theta}(\tau )||\, \mathrm{d}\tau \right)
\end{equation}
where $T$ represents the duration of the desired trajectory $\bm{r}_d(\va,\,t)$, $\mathcal{A}$ is a feasible set for the parameter vector $\bm{a}$ (which is the optimization variable), and $||\cdot||$ a matrix norm. Note that the initial parameter vector $\va$ gets preconditioned: $(i)$ to set the time and position of the last way-point $(t_T,\, \bm{\mathcal{P}}_T)$; $(ii)$ to take the uncertain behavior of the control into account by applying an offset to $\bm{\mathcal{P}}_T$. {This is done through a short optimization}{This is done through a short optimization with an equality constraint, which forces the last way-point to be placed in a way that the simulated system (in the nominal case where $\bm{p} =\bm{p}_c$) with its inaccurate controller goes to the actual target when following the reference trajectory.}
The rationale behind \equref{opt1} is as follows: $(i)$ the first term in \equref{opt1} aims at minimizing the state sensitivity at the final time $T$, so that the tracking accuracy of $\bm{r}_d(\va,\,t)$ at $t=T$ is made most insensitive to uncertainties in the model parameters; $(ii)$ the second term in \equref{opt1} aims at minimizing the input sensitivity during the whole trajectory, in order to obtain control inputs that are most insensitive (i.e., with minimal deviations) against variations of the robot parameters. The quantities $w_1$ and $w_2$ are suitable weights to combining these two objectives in a single scalar cost.

==> 220_observability.tex <==
%Returning to the generic robot model of \secref{control}, which defined the system dynamics $\vf$, the state vector $\vx$, and the control inputs $\vu$, we noticed that the 
In any non-trivial case, the control action of a robot needs an accurate knowledge of its state $\vx$ at run-time. This can pose a problem as many states are often not directly measurable through, \eg, exteroceptive sensors. Online state estimation is one way of making the state vector $\vx$ available by iteratively building an estimation of it. This is possible through the system model ($\vf$) and the comparison of sensor measurements with system state-based measurement models $\vh\in\mathbb{R}^{n_h}$ (output),  \cite{weiss_versatile_2012,hausman_self-calibrating_2016,boehm_filter_2021}. %In a repeating loop of state change predictions based on the system dynamics $\vf$ and control inputs $\vu$, and the update of those predictions through the sensor measurements, one can get an estimate of the systems state.

A so-called observability analysis, \cite{hermann_nonlinear_1977,krener_measures_2009,kelly_visual-inertial_2011}, can be used to see if a certain system model and sensor measurement combination makes the state vector $\vx$ observable (meaning it can be estimated). How well such estimates perform depends on the accuracy of the system model and sensors used, but equally important on the particular control inputs given to the robot.

\subsection{Quality of Observability}

A state is well observable if the system output changes significantly by slightly perturbing the state \cite{hermann_nonlinear_1977, krener_measures_2009}. This is the idea of quality of observability and based on it \cite{preiss_simultaneous_2018,hausman_observability-aware_2017} proposed the \gls{e2log} to evaluate the quality of observability of a whole trajectory $\bm{r}_d(\va,\,t)$ with a duration $T$.

The first step is to calculate the Lie Derivatives of our system model according to
\begin{equation}
    \begin{gathered} 
        \label{eq:lie_derivatives}   
        \Lie{0}{}\vh = \vh\left(\vx,\vu\right) \in \mathbb{R}^{n_h \times 1}, \\
        \Lie{i}{\vf}\vh = \tfrac{\partial\left(\Lie{i-1}{\vf}\vh\right)}{\partial\vx}\vf(\vx,\vu) \in \mathbb{R}^{n_h \times 1}.
    \end{gathered}
\end{equation}
These Lie Derivatives allow for an $n$-th order Taylor expansion that approximates the Jacobian matrix of the sensor model $\vh$ around a point in time $t_0$ with $\delta{t} = t-t_0$, giving
\begin{equation}
    \label{eq:taylor_approximation}
    \left.\frac{\partial}{\partial \vx}\vh_{}(\vx(t), \vu(t)) \right|_{t_0} = \sum_{i=0}^n \frac{\delta{t}^i}{i!}\nabla \Lie{i}{\vf}\vh \in \mathbb{R}^{n_h \times n_x}.
\end{equation}
This approximation models the sensitivity of the output/measurements with respect to the control inputs, the state and its changes. The latter is part of this sensitivity metric because of the high-order Lie derivatives adding the system dynamics to the approximation.
This sensitivity formulation applied to a whole trajectory $\bm{r}_d(\va,\,t)$ over the duration of $T$ allows us to calculate the quality of observability along the trajectories.

Over a short time horizon $H$, one is able to calculate the state sensitivity of this segment by integrating the input-output map $\vK$ of measurement models and system dynamics, giving
\begin{equation}
    \begin{gathered} 
        \label{eq:e2log_piece}
        \widetilde{\vW}_{t_0,H}(\va) = \int_0^H \vK_{\va,t_0} (t_0 + t)^\transpose \vK_{\va,t_0} (t_0 + t) dt,\\ 
        \vK_{\va, t_0} (t) = \left.\frac{\partial}{\partial \vx}\vh_{}(\vx_\va(t), \vu_\va(t)) \right|_{t_0}.
    \end{gathered}
\end{equation}
Note that $\vx_\va(t)$ and $\vu_\va(t)$ are the state values and control inputs based on the trajectory parametrization of $\va$.
To balance different magnitudes of state values in $\vx$, a column scaling can be applied $\vK_{}^{'} = \vK\,\diag(\vs)^{\inverse}$ with $\vs$ containing standard deviation values of each state received from empirical evaluations of the estimation process \cite{preiss_simultaneous_2018}.

Summing all these quality measure segments along the trajectory $\bm{r}_d(\va,\,t)$ gives us the \gls{e2log}
\begin{equation}
    \label{eq:e2log}
    \widetilde{\vW}_{\cO}(\va) = \sum_{k=0}^{N} \widetilde{\vW}_{k\Delta t,\Delta t}(\va)  \in \mathbb{R}^{n_x \times n_x}
\end{equation}
with $\Delta t = \tfrac{T}{N}$ and $N$ the number of segments {over the whole trajectory}, which is an empirical parameter and is usually set as high as possible while being aware of the impact on the computation times \cite{preiss_simultaneous_2018}.

One can see that the estimation performance is not only influenced by its state but also by the control inputs  $\vu$.

\subsection{Observability-aware Optimization}

Observability-aware trajectories are generated by putting $\widetilde{\vW}_{\cO}(\va)$ as the cost function into an optimization problem with the trajectory parameters $\va$ as the optimization variable. In this paper's formulation the objective is to improve the least sensitive state (or combination of states) through the smallest eigenvalue of $\widetilde{\vW}_{\cO}(\va)$. Adding a minus to this value gives us the possibility to use it in an minimization problem with the objective function $\bm{\Lambda}(\va) = -\sigma_{\min}(\widetilde{\vW}_{\cO}(\va))$, thus
\begin{equation}
    \label{eq:e2log_optimization}
    \bm{a}_{opt} = \arg \, \underset{\bm{a} \in \mathcal{A}}{\min}\ \bm{\Lambda}(\va)
\end{equation}
% \begin{align}
%     \begin{split}
%         \label{eq:e2log_optimization}
%         \underset{\theta}{\text{maximize}} \quad & \sigma_{\min}(\widetilde{\vW}_{\cO}(\theta)) \\
%         \text{subject to} \quad
%         & \theta\ \text{suitable for task} \\
%         & \theta\ \text{dynamically feasible}
%     \end{split}
% \end{align}
% The optimization is often subject to inequality constraints that keep the trajectory within bounding boxed and prevent it from exceeding dynamic limitations.

% For later use we convert the maximization into a minimization by switching the sign of the cost, $-\sigma_{\min}(\widetilde{\vW}_{\cO}(\theta))$, and try to minimize the negative smallest eigenvalue.

This optimization results in a trajectory with the best possible observability properties, improving the states convergence by lowering the uncertainty and increasing the overall accuracy.
With the \gls{e2log} estimator-implementation, agnostic observability-aware trajectories can be generated for a variety of systems.

\subsection{Estimation Model \& Properties}
\label{sec:estimation_model}

The state estimation and, therefore, the derivation of the observability-aware trajectory optimization for the quadrotor \gls{uav} in this paper is based on the \gls{iekf} state estimation implementation presented in \cite{boehm_filter_2021} and is new for rigid body dynamics based system models. Following this work, the squared rotor speeds as control inputs need to be substituted with ${\vu^{*} = \left[ u_1, u_2, u_3, u_4 \right]_{}^{\transpose}}$ to make further calculations (the approximation in \equref{taylor_approximation}) possible.
This previous work shows that it is possible to estimate the thrust force and drag moment coefficients, $k_f$ and $k_m$. The estimation only needs rotor speed input, pose sensor and \gls{imu} measurements, and few a prior measurements of the quadrotor.

% \textcolor{red}{Parameters of Quadrotor! What do we need to add to Pascal's model.}


% Deltas compared to Pascal's control model!
% \begin{itemize}
%     \item Short description on states, dynamics and measurement models
%     \item Write the observability properties of Hummingbird, reference to paper for others
%     \item Resulting "constraints" and what to expect
% \end{itemize}


==> figures/confidenc_ellipse_plot.tex <==
\begin{figure}[b]   
    % \vspace{-2em}
    \centering
    \begin{tikzpicture}
        \node[inner sep=0] (image) at (0,0) {\includegraphics[width=0.3\columnwidth]{figures/pdfs/tracking_error_ellipse_XY_old.pdf}};
        \draw[red,ultra thick] (image.south east) -- (image.north west);
        \draw[red,ultra thick] (image.north east) -- (image.south west);
        \draw[red,ultra thick] (image.south west) rectangle (image.north east);
    \end{tikzpicture}
    \begin{tikzpicture}
        \node[inner sep=0] (image) at (0,0) {\includegraphics[width=0.3\columnwidth]{figures/pdfs/tracking_error_ellipse_XZ_old.pdf}};
        \draw[red,ultra thick] (image.south east) -- (image.north west);
        \draw[red,ultra thick] (image.north east) -- (image.south west);
        \draw[red,ultra thick] (image.south west) rectangle (image.north east);
    \end{tikzpicture}
    \begin{tikzpicture}
        \node[inner sep=0] (image) at (0,0) {\includegraphics[width=0.3\columnwidth]{figures/pdfs/tracking_error_ellipse_YZ_old.pdf}};
        \draw[red,ultra thick] (image.south east) -- (image.north west);
        \draw[red,ultra thick] (image.north east) -- (image.south west);
        \draw[red,ultra thick] (image.south west) rectangle (image.north east);
    \end{tikzpicture}
    \caption{\revisionchange{For each trajectory, we show the 90\% confidence ellipse associated to the point cloud of the final outputs $\vr_i(T)$, with $\delta \vp = 10\%$. The comparison supports the insights of \figref{convergence} and \figref{tracking} as the smallest ellipse is due to the \gls{sis} optimized and the biggest due to the \gls{e2log} optimized trajectory.}{}}
    \label{fig:ellipse} 
\end{figure}
